Full-Program Induction: Verifying Array Programs sans Loop Invariants

Arrays are commonly used in a variety of software to store and process data in loops. Automatically proving safety properties of such programs that manipulate arrays is challenging. We present a novel verification technique, called full-program induction, for proving (a sub-class of) quantified as well as quantifier-free properties of programs manipulating arrays of parametric size $N$. Instead of inducting over individual loops, our technique inducts over the entire program (possibly containing multiple loops) directly via the program parameter $N$. The technique performs non-trivial transformations of the given program and pre-conditions during the inductive step. The transformations assist in effectively reducing the assertion checking problem by transforming a program with multiple loops to a program which has fewer and simpler loops or is loop-free. Significantly, full-program induction does not require generation or use of loop-specific invariants. To assess the efficacy of our technique, we have developed a prototype tool called Vajra. We demonstrate the performance of Vajra vis-a-vis several state-of-the-art tools on a large set of array manipulating benchmarks from the international software verification competition (SV-COMP) and on several programs inspired by algebraic functions that perform polynomial computations.

==> ex-ss-intro.tex <==
\begin{table*}[h!]
\caption{(a) Program $\PP_N$, (b) Program $\PP_N$ after renaming, (c)
  Program $\PP_{N-1}$ and (d) Difference Program $\partial \PP_N$}
\label{tab:ex-ss-intro}
\begin{tabular} { p{7.6cm}  p{6.6cm} }
\begin{alltt}
// assume(\(\forall\)i\(\in\)[0,N) A[i] = 1)

1.  S = 0;
2.  for(i=0; i<N; i++) \{
3.    S = S + A[i];
4.  \}

5.  for(i=0; i<N; i++) \{
6.    A[i] = A[i] + S;
7.  \}

8.  for(i=0; i<N; i++) \{
9.    S = S + A[i];
10. \}

// assert(S = N \(\times\) (N+2))
\end{alltt}
  &
\begin{alltt}
// assume(\(\forall\)i\(\in\)[0,N) A[i] = 1)

1.  S = 0;
2.  for(i=0; i<N; i++) \{
3.    S = S + A[i];
4.  \}

5.  for(i=0; i<N; i++) \{
6.    A1[i] = A[i] + S;
7.  \}

8.  S1 = S;
9.  for(i=0; i<N; i++) \{
10.   S1 = S1 + A1[i];
11. \}

// assert(S1 = N \(\times\) (N+2))
\end{alltt}
\\
\begin{center}(a)\end{center}
&
\begin{center}(b)\end{center}
\\
\begin{alltt}
// assume(\(\forall\)i\(\in\)[0,N-1) A[i] = 1)

1.  S_Nm1 = 0;
2.  for(i=0; i<N-1; i++) \{
3.    S_Nm1 = S_Nm1 + A[i];
4.  \}

5.  for(i=0; i<N-1; i++) \{
6.    A1_Nm1[i] = A[i] + S_Nm1;
7.  \}

8.  S1 = S;
9.  for(i=0; i<N-1; i++) \{
10.   S1_Nm1 = S1_Nm1 + A1_Nm1[i];
11. \}

// assert(S1_Nm1 = (N-1) \(\times\) (N+1))
\end{alltt}
&
\begin{alltt}
// assume(N>1 \(\wedge\) A[N-1] = 1 \(\wedge\) S_Nm1 = N-1
//  \(\wedge\) \(\forall\)i\(\in\)[0,N-1) A1_Nm1[i] = N
//  \(\wedge\) S1_Nm1 = (N-1) \(\times\) (N+1))

1.  S = S_Nm1 + A[N-1];

2.  for(i=0; i<N-1; i++) \{
3.    A1[i] = A1_Nm1[i] + 1;
4.  \}
5.  A1[N-1] = A[N-1] + S;

6.  S1 = S1_Nm1 + A[N-1];
7.  S1 = S1 + (N-1);
8.  S1 = S1 + A1[N-1];

// assert(S=N \(\wedge\)
//  \(\forall\)i\(\in\)[0,N) A1[i] = N+1
//  \(\wedge\) S1 = N \(\times\) (N+2))
\end{alltt}
\\
\begin{center}(c)\end{center}
&
\begin{center}(d)\end{center}
\\
\end{tabular}
\end{table*}


==> ex-ss-ssa.tex <==
%% \begin{wrapfigure}[20]{r}{0.38\textwidth}
%% \vspace{-2ex}

\begin{figure*}[tb]
  \begin{minipage}{0.12\linewidth}
    ~
  \end{minipage}
\begin{minipage}{0.38\linewidth}
\begin{alltt}
// assume(\(\forall\)i\(\in\)[0,N) A[i] = 1)

1.  S = 0;
2.  for(i=0; i<N; i++) \{
3.    S = S + A[i];
4.  \}
{\color{blue}
// Lines 5-7 are glue code
5.  S1 = S;
6.  for(i=0; i<N; i++)
7.    A1[i] = A[i];}
8.  for(i=0; i<N; i++) \{
9.    A1[i] = A1[i] + S1;
10. \}
{\color{blue}
// Lines 11-13 are glue code
11.  S2 = S1;
12.  for(i=0; i<N; i++)
13.    A2[i] = A1[i];}
14.  for(i=0; i<N; i++) \{
15.   S2 = S2 + A2[i];
16. \}

// assert(S2 = N \(\times\) (N+2))
\end{alltt}
\begin{center}
  (a)
\end{center}
\end{minipage}
\begin{minipage}{0.38\linewidth}
\begin{alltt}
// assume(\(\forall\)i\(\in\)[0,N) A[i] = 1)

1.  S = 0;
2.  for(i=0; i<N; i++) \{
3.    S = S + A[i];
4.  \}





5.  for(i=0; i<N; i++) \{
6.    A1[i] = A[i] + S;
7.  \}

{\color{blue}
// Optimized glue code
8.  S1 = S;}

9.  for(i=0; i<N; i++) \{
10.   S1 = S1 + A1[i];
11. \}

// assert(S1 = N \(\times\) (N+2))
\end{alltt}
\begin{center}
  (b)
\end{center}
\end{minipage}
\begin{minipage}{0.1\linewidth}
  ~
\end{minipage}
%% \begin{minipage}{0.44\linewidth}
%% \caption
%% { Program after renaming the variables and arrays.  New name has been
%%   introduced for the array updated in the second loop as we want to
%%   distinguish its value from the array in the pre-condition.
%%   Similarly, the scalar in the last loop is also renamed so that we
%%   can distinguish it from the scalar being updated in the first loop.
%%   Notice that variables referred in the post-condition are also
%%   renamed accordingly.  }
%% \end{minipage}
\caption{Renaming (a) Unoptimized and (b) Optimized}
\label{fig:ss-ssa}
\end{figure*}

%% \end{wrapfigure}

